Energy-conserving formulation of the two-fluid model for incompressible two-phase flow in channels and pipes

We show that the one-dimensional (1D) two-fluid model (TFM) for stratified flow in channels and pipes (in its incompressible, isothermal form) satisfies an energy conservation equation, which arises naturally from the mass and momentum conservation equations that constitute the model. This result extends upon earlier work on the shallow water equations (SWE), with the important difference that we include non-conservative pressure terms in the analysis, and that we propose a formulation that holds for ducts with an arbitrary cross-sectional shape, with the 2D channel and circular pipe geometries as special cases. The second novel result of this work is the formulation of a finite volume scheme for the TFM that satisfies a discrete form of the continuous energy equation. This discretization is derived in a manner that runs parallel to the continuous analysis. Due to the non-conservative pressure terms it is essential to employ a staggered grid, which requires careful consideration in defining the discrete energy and energy fluxes, and the relations between them and the discrete model. Numerical simulations confirm that the discrete energy is conserved.

==> control_volume_schematic_two-fluid_multi.tex <==
\begin{tikzpicture}[scale=1.35, baseline=(current bounding box.north)]

% Wave and bottom of box (liquid area)
%\filldraw[fill=blue!30!white, draw=black] (-2,0) sin (-1,0.25) cos (0,0) sin (1,-0.25) cos (2,0) -- (2,-1.25) -- (-2,-1.25) -- cycle;
%\filldraw[fill=blue!30!white, draw=black] (-2,1.25) -- (2,1.25) -- (2,-1.25) -- (-2,-1.25) -- cycle;
%\filldraw[fill=blue!30!white, draw=black] (-2,0) sin (-1,0.25) cos (0,0) sin (1,-0.25) cos (2,0) -- (2,-1.25) -- (-2,-1.25) -- cycle;
\filldraw[fill=blue!30!white, draw=black] (-2,0) sin (-1,0.25) cos (0,0) sin (1,-0.25) cos (2,0) sin (3,0.25) cos (4,0) -- (4,-1.25) -- (-2,-1.25) -- cycle;

% Box Length
%\draw[thick, -{Latex[width = 2.2mm, length = 2.2mm]}] (-2.75, -1.25)--(3,-1.25);
%\draw[thick, -{Latex[width = 2.2mm, length = 2.2mm]}] (2.75, -1.25)--(-3,-1.25);
%\node [below] at (0,-1.25) {$L$};
\draw[-{Latex[width = 2.2mm, length = 2.2mm]},dashed] (-2.02, -1.45)--(2.5,-1.45);
%\node [below] at (2.3,-1.45) {$s$};
\node [right] at (2.5,-1.45) {$s$};

\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (-0.5, -0.8)--(0.75,-0.8);
\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (0.5,-0.8) --(-0.75, -0.8);
\node [below] at (0,-0.8) {$\delta s$};
%\node [below] at (-0.75,-1.45) {$s_1$};
%\node [below] at (0.75,-1.45) {$s_2$};


\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (4.15, -1)--(4.15,1.25);
\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (4.15,1)--(4.15, -1.25);
\node [right] at (4.15,0) {$H$};
\draw[-{Latex[width = 2.2mm, length = 2.2mm]},dashed] (-2.2, -1.32)--(-2.2,0.8);
\node [left] at (-2.2,0.6) {$h$};
%\node [above] at (-2.2,0.625) {$h$};



% Box
%\draw[thick] (-2,-1.25) rectangle (2,1.25);
\draw[thick] (-2,-1.25) rectangle (4,1.25);



% Control Volume
\draw[scale=1,domain=-0.75:0.75,smooth,variable=\x, thick, dashed] plot ({\x},{-0.25*sin((2*pi/4)*\x r)-0.05}) -- (0.75,-1.2) -- (-0.75,-1.2) -- (-0.75,0.181) -- cycle;
\draw[scale=1,domain=-0.75:0.75,smooth,variable=\x, thick, dashed] plot ({\x},{-0.25*sin((2*pi/4)*\x r)+0.05}) -- (0.75,1.2) -- (-0.75,1.2) -- (-0.75,0.281) -- cycle;

%\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (-0.75, 0.75)--(-1.15,0.75);
%\node [below] at (-0.95,0.75) {$\v{n}_U$};
%\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (0.75, 0.75)--(1.15,0.75);
%\node [below] at (0.95,0.75) {$\v{n}_U$};

%\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (-0.75, -0.75)--(-1.15,-0.75);
%\node [above] at (-0.95,-0.75) {$\v{n}_L$};
%\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (0.75, -0.75)--(1.15,-0.75);
%\node [above] at (0.95,-0.75) {$\v{n}_L$};

%\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (0, -1.2)--(0,-1.6);
%\node [right] at (0,-1.35) {$\v{n}_L$};
%\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (0, 1.2)--(0,1.6);
%\node [right] at (0,1.4) {$\v{n}_U$};

%\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (0, 0)--(0.0943,0.377);
%\node [right] at (0.04715,0.1886) {$\v{n}_L$};
%\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (0, 0)--(-0.0943,-0.377);
%\node [left] at (-0.04715,-0.1886) {$\v{n}_U$};

%\node at (0,0) {$\begin{aligned} \int_V \rho \, \mathrm{d} v \\ V \\ \int_V \rho \v{u} \, \mathrm{d} v \end{aligned}$};
\node at (0,0.65) {$ \Omega_U$};
\node at (0,-0.45) {$ \Omega_L$};

% velocity
%\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (1.1, -0.4)--(1.7,-0.4);
%\node [below] at (1.4,-0.4) {$u$};
%\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (-1.6, -0.85)--(-1.6,-0.25);
%\node [left] at (-1.6,-0.5) {$u_3$};

% Gravity
%\draw[thick, -{Latex[width = 2.2mm, length = 2.2mm]}] (2.4, 1.1)--(2.208,-1.09);
%\draw[dashed] (2.4, 1.1)--(2.4,-1.1);
%\node [left] at (2.295,0) {$\v{g}$};
%\centerarc[](2.4,1.1)(-90:-95:2)
%\node at (2.31,-0.8) {$\phi$};

%\draw[thick, -{Latex[width = 2.2mm, length = 2.2mm]}] (2.25, 1.1)--(2.25,-1.1);
%\node [right] at (2.25,0) {$\v{g}$};

 %%%%\node [left] at (3,-1.01) {$\phi$};
 


%\draw[thick, -{Latex[width = 2.2mm, length = 2.2mm]}] (0, 0)--(0.3617,-0.142);
%\node [below] at (0.18,-0.07) {$\v{t}$};

\draw[] (-2.2,-1.45) circle (0.13); %-2.5 -1.7 % 0.75 0.575
\draw[] (-2.292,-1.358) -- (-2.108,-1.542);
\draw[] (-2.108,-1.358) -- (-2.292,-1.542);
\node [left] at (-2.292,-1.45) {$y$};

% Profile
%\draw[black] plot[smooth, domain=0:1] (-0.5 * \x * \x +0.5, \x);
\draw[black] plot[smooth, domain=0.25:1.25, variable=\y] ({-1.5*(\y-0.6)*(\y-0.6)+0.5+0.18375+3-0.5},{\y});
\draw[dashed] (2.55,-1.25)--(2.55,1.25);
\draw[black] (2.55,-1.25)--(3,0.25);
\draw[-{Latex[width = 1mm, length = 1mm]}] (2.55, -1)--(2.625,-1);
\draw[-{Latex[width = 1mm, length = 1mm]}] (2.55, -0.75)--(2.7,-0.75);
\draw[-{Latex[width = 1mm, length = 1mm]}] (2.55, -0.5)--(2.775,-0.5); 
\draw[-{Latex[width = 1mm, length = 1mm]}] (2.55, -0.25)--(2.85,-0.25); \node [right] at (2.85,-0.25) {$u'$};
\draw[-{Latex[width = 1mm, length = 1mm]}] (2.55, 0)--(2.925,0);
\draw[-{Latex[width = 1mm, length = 1mm]}] (2.55, 0.25)--(3,0.25);
\draw[-{Latex[width = 1mm, length = 1mm]}] (2.55, 0.5)--(3.1688,0.5);
\draw[-{Latex[width = 1mm, length = 1mm]}] (2.55, 0.75)--(3.15,0.75);
\draw[-{Latex[width = 1mm, length = 1mm]}] (2.55, 1)--(2.9438,1);

% Interface height
\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (2, -0.625)--(2,-1.25);
\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (2, -0.625)--(2,0);
\node [left] at (2,-0.625) {$H_L$};

% Gas height
\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (2, 0.625)--(2,0);
\draw[-{Latex[width = 2.2mm, length = 2.2mm]}] (2, 0.625)--(2,1.25);
\node [left] at (2, 0.625) {$H_U$};

%% Cross section
%\filldraw[fill=blue!30!white, draw=black] (-3.9798,-0.2) -- (-2.0202,-0.2) arc (-11.087:-168.913:1) -- cycle;
\filldraw[fill=blue!30!white, draw=black] (-5.2267,-0.2404) -- (-2.7733,-0.2404) arc (-11.087:-168.913:1.25) -- cycle;
\draw[thick] (-4,0) circle (1.25);

%% Control volumes
%\draw[dashed] (-4,0) circle (1.2);
%\draw [dashed] (-5.17378,-0.2494) -- (-2.82622,-0.2494) arc (-12:-168:1.2) -- cycle;
\draw [thick, dashed] (-5.1644,-0.2903) -- (-2.8356,-0.2903) arc (-14:-166:1.2) -- cycle;
\draw [thick, dashed] (-5.1852,-0.1877) -- (-2.8148,-0.1877) arc (-9:189:1.2) -- cycle;

\node at (-4,-0.6) {$\Omega_L$};
\node at (-4,0.6) {$\Omega_U$};

%% Coordinates
\draw[] (-5.35,-1.45) circle (0.13); 
%\draw[] (-5.4419,-1.5419) -- (-5.2581,-1.3581);
%\draw[] (-5.4419,-1.3581) -- (-5.2581,-1.5419);
\filldraw[fill=black, draw=black] (-5.35,-1.45) circle (0.03); 
\node [left] at (-5.415,-1.45) {$s$};

\draw[-{Latex[width = 2.2mm, length = 2.2mm]},dashed] (-5.35, -1.32)--(-5.35,0.8);
\node [left] at (-5.35,0.6) {$h$};

\draw[-{Latex[width = 2.2mm, length = 2.2mm]},dashed] (-5.22, -1.45)--(-3.45,-1.45);
\node [right] at (-3.45,-1.45) {$y$};

\end{tikzpicture}
